Multi-Criteria Dimensionality Reduction with Applications to Fairness

Dimensionality reduction is a classical technique widely used for data analysis. One foundational instantiation is Principal Component Analysis (PCA), which minimizes the average reconstruction error. In this paper, we introduce the "multi-criteria dimensionality reduction" problem where we are given multiple objectives that need to be optimized simultaneously. As an application, our model captures several fairness criteria for dimensionality reduction such as our novel Fair-PCA problem and the Nash Social Welfare (NSW) problem. In Fair-PCA, the input data is divided into $k$ groups, and the goal is to find a single $d$-dimensional representation for all groups for which the minimum variance of any one group is maximized. In NSW, the goal is to maximize the product of the individual variances of the groups achieved by the common low-dimensional space. Our main result is an exact polynomial-time algorithm for the two-criterion dimensionality reduction problem when the two criteria are increasing concave functions. As an application of this result, we obtain a polynomial time algorithm for Fair-PCA for $k=2$ groups and a polynomial time algorithm for NSW objective for $k=2$ groups. We also give approximation algorithms for $k>2$. Our technical contribution in the above results is to prove new low-rank properties of extreme point solutions to semi-definite programs. We conclude with experiments indicating the effectiveness of algorithms based on extreme point solutions of semi-definite programs on several real-world data sets.

==> macro-tao.tex <==
% %-------PAGE FORMATTING-------
% %
% %\usepackage[margin=1in]{geometry}
% %       \addtolength{\oddsidemargin}{-.5in}
% %       \addtolength{\evensidemargin}{-.5in}
% \usepackage{geometry}
% \geometry{top=1.25in}
% \geometry{bottom=1.25in}
% \geometry{left=1.25in}
% \geometry{right=1.25in}
%
% %-------PACKAGES-------
% %\usepackage{mathptmx} %for the smaller font
% %\usepackage{anysize}
% %\marginsize{1in}{1in}{1in}{1in}
% %\usepackage{styles/title}
% %\usepackage{styles/ack}
% \usepackage{latexsym}
% %\usepackage{algorithm}
% %\usepackage{algorithmic}
% \usepackage{amsmath}
% \usepackage{amsfonts}
% %\usepackage{amsthm}
% \usepackage{amssymb}
% \usepackage{bbm}
% %\usepackage{bbold}
% %\usepackage{epsfig}
% \usepackage{tabls}
% \usepackage{theorem}
% \usepackage[dvips]{graphicx}
% \usepackage{color}
% \usepackage{enumerate}
% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}
% %\newcommand{\kdchange}[0]{\marginpar{\tiny\bf KD}}
% \newcommand{\ignore}[1]{}
% \usepackage{sansmath}
% %\usepackage{fontds}
% \usepackage{hyperref}
% \usepackage{array}
%
% %------SPECIAL FORMATTING COMMANDS--------
% \newcolumntype{x}[1]{>{\centering\arraybackslash\hspace{0pt}}p{#1}}
%
% %---------COMMENTS------------
% \newcommand{\ms}[1]{\color{red} Mohit's Comment: {#1} \color{black}}
% \newcommand{\Tao}[1]{\color{green} Tao's Comment: {#1} \color{black}}
% \newcommand{\Todo}[1]{\color{blue} [TO-DO: {#1}] \color{black}}
 \newcommand{\cut}[1]{}
%
%
% %-------MATH OPERATORS-------
% \newcommand{\poly}{\operatorname{poly}}
% \newcommand{\polylog}{\operatorname{polylog}}
% \newcommand{\Opt}{\textup{Opt}}
% \newcommand{\Obj}{\textup{Obj}}
% \newcommand{\Prob}[2]{\underset{#1}{\ensuremath{\mathsf{Pr}}}\left[#2\right]}
% \newcommand{\Ex}[2]{\underset{#1}{\mathbb{E}} \left[ #2  \right]}
% \newcommand{\NP}{\mathsf{NP}}
% \newcommand{\oneIn}{\mathbbm{1}}
%
% %-------FIXED-SIZED DEMILITORS-------
% \newcommand{\paren} [1] {\ensuremath{ \big( {#1} \big) }}
% \newcommand{\bigparen} [1] {\ensuremath{ \Big( {#1} \Big) }}
% %\newcommand{\set}[1]{\ensuremath{\{ #1 \}}}
%
% %-------AUTO-SIZED DELIMITORS-------
% \newcommand{\abs}[1]{\left|#1\right|}
% \newcommand{\size}[1]{\ensuremath{\left|#1\right|}}
%
\newcommand{\br}[1]{\left[#1\right]}
\newcommand{\pr}[1]{\left(#1\right)}
\newcommand{\bc}[1]{\left\{#1\right\}}
\renewcommand{\set}[1]{\ensuremath{\left\{#1\right\}}}
\newcommand{\an}[1]{\left\langle#1\right\rangle}
%
% \newcommand{\ceil}[1]{\ensuremath{\left\lceil#1\right\rceil}}
\newcommand{\floor}[1]{\ensuremath{\left\lfloor#1\right\rfloor}}
% \newcommand{\norm}[2]{\ensuremath{\Vert {#1} \Vert_{#2}}}
% %\newcommand{\norm}[1]{\left|\left|#1\right|\right|}
% \newcommand{\norme}[1]{\norm{#1}_2}
%
% %-------FUNCTIONS DELIMITORS--------
% \newcommand{\expct}[1]{\ensuremath{\text{{\bf E}$\left[#1\right]$}}}
% \newcommand{\Cov}[1]{\operatorname{Cov}\pr{#1}}
% \newcommand{\Var}[1]{\operatorname{Var}\pr{#1}}
% \newcommand{\sgn}[1]{\textup{sgn}\pr{#1}}
% \newcommand{\tr}[1]{\operatorname{tr}\pr{#1}}
% %\newcommand{\argmin}{\operatorname*{argmin}}
% %\newcommand{\argmax}{\operatorname*{argmax}}
% \def\argmax{\operatornamewithlimits{arg\,max}}
% \def\argmin{\operatornamewithlimits{arg\,min}}
% \newcommand{\prob}[1]{\ensuremath{\text{{\bf Pr}$\left[#1\right]$}}}
% \newcommand{\E}[1]{\ensuremath{\text{{\bf E}$\left[#1\right]$}}}
% %\newcommand{\Prob}[2]{\underset{#1}{\capPr} \left[#2\right]}
% %\newcommand{\E}[2]{\underset{#1}{\mathbb{E}} \left[ #2 \right]}
% \newcommand{\VCD}[1]{\text{VCDim}\left( #1 \right)}
% \newcommand{\Rec}[1]{\text{Rec}\left( #1 \right)}

% % Symbols, Sets, and Values
% % ---------------------------------------------
% \newcommand{\true}{{\sf true}\xspace}
% \newcommand{\false}{{\sf false}\xspace}
% \newcommand{\OPT}[0]{{\ensuremath{\sf{OPT}}}}
% \newcommand{\CP}[0]{{\ensuremath{\sf{CP}}}}
% \newcommand{\Alg}[0]{{\ensuremath{\sf{Alg}}}}
% \newcommand{\distrib}[0]{{\ensuremath{\mathcal{D}}}}
% \newcommand{\family}[0]{{\ensuremath{\mathcal{F}}}}
% \newcommand{\cover}[0]{{\ensuremath{\mathcal{C}}}}
% \newcommand{\instance}[0]{{\ensuremath{\mathcal{I}}}}
% \newcommand{\minimize}{\mbox{\rm minimize }}
% \newcommand{\maximize}{\mbox{\rm maximize }}
% \newcommand{\st}{\mbox{\rm subject to }}
\newcommand{\diag}{\textup{diag}}
% \newcommand{\comps}{\ensuremath{{\cal C}}}
% \newcounter{obs}
% \stepcounter{obs} \ignore{
% \definecolor{back-high}{rgb}{1,1,0.6}
% \definecolor{back}{rgb}{1,1,.5}
% \definecolor{nc}{rgb}{.38,.5,.9}
% \definecolor{nc2}{rgb}{.3,.8,.3}
% \definecolor{db}{rgb}{0,0,.3}
% \definecolor{dr}{rgb}{1,0.5,0}
% \definecolor{bg}{rgb}{1,.5,.2}
% \definecolor{bg2}{rgb}{1,1,.5}
% \definecolor{bgs}{rgb}{.5,1,.5}
% \definecolor{mc1}{rgb}{.7,.7,1}
% \definecolor{mc2}{rgb}{.8,.8,1}
% \definecolor{bgslight}{rgb}{.8,1,.8}
% }
%
% %\addtolength{\parskip}{-0.5mm}
% %-------ENVIRONMENT-------
% \DeclareMathAlphabet{\altmathcal}{OMS}{cmsy}{m}{n}
%
% \newtheorem{fact}{Fact}[section]
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{corollary}[theorem]{Corollary}
% \newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{definition}[theorem]{Definition}
% \newtheorem{claim}[theorem]{Claim}
% \newtheorem{observation}[theorem]{Observation}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{quest}{Question}
% \newenvironment{proof}{\smallskip\noindent{\bf Proof}:}{$\hfill % \Box$\\}
% \newenvironment{proofsketch}{\smallskip\noindent{\bf Proof Sketch}:}{$\hfill \Box$\\}
% \newenvironment{proofof}[1]{\smallskip\noindent{\bf Proof of #1}:}{$\hfill \Box$\\}
%
%
% %--------SYMBOLS---------
% \def\bsq{$\blacksquare$}
% \def\A{\mathcal{A}}
% \def\i{\mathcal{I}}
% \def\P{\mathcal{P}}
% \def\I{\mathcal{I}}
% \def\M{\mathcal{M}}
\def\RR{\mathbb{R}}
% \def\BB{\altmathcal{B}}
% \def\Z{\mathbb{Z}}
% \def\Q{\mathbb{Q}}
% \def\U{\altmathcal{U}}
% \def\e{\mathbf{e}}
% \def\SS{\altmathcal{S}}
% \def\h{h}
% \def\l{\ell}
% \newcommand{\sbq}{\subseteq}
% \newcommand{\spq}{\supseteq}
% \renewcommand{\v}{{\mathbf{v}}} \renewcommand{\u}{{\mathbf{u}}}
% \renewcommand{\M}{{\mathcal{M}}}
% \newcommand{\A}{{\mathcal{A}}}
% \newcommand{\SO}{{\mathcal{SO}}}
% \newcommand{\st}{\mbox{\rm s.t. }}
%
% %\begin{document}
% \def \I   {{\mathcal I}}
%
%
% \def \CC   {{\mathbb C}}
% \def \FF   {{\mathbb F}}
% \def \SS   {{\mathbb S}}
% \def \DD   {{\mathbb D}}
% \def \PP   {{\mathbb P}}
% \def \RR   {{\mathbb R}}
% \def \II   {{\mathbb I}}
% \def \EE   {{\mathcal E}}
% \def \TT   {{\mathbb T}}
\def \OPT  {\mbox{\rm OPT}}
% \def \m   {{\mathbb M}}
% \def \M   {{\mathcal M}}
% \def \I   {{\mathcal I}}
% \def \A   {{\mathcal A}}
% \def \mZ  {{\mathbb Z}}
% \def \N   {{\mathcal N}}
% \def \H   {{\mathcal H}}
% \def \C   {{\mathcal C}}
% \def \B   {{\mathcal B}}
% \def \ZZ   {{\mathbb Z}}
\def \sdp {\mathbb{SDP(I)}}
\def \sdpII {\mathbb{SDP(II)}}
\def \sdpa {\mathbb{SDP}}
\def \sdpr {\mathbb{SDP}(r)}

\newcommand{\tao}[1]{\textbf{\color{green}[tao: #1]}}



